A Survey of Orthographic Information in Machine Translation

Machine translation is one of the applications of natural language processing which has been explored in different languages. Recently researchers started paying attention towards machine translation for resource-poor languages and closely related languages. A widespread and underlying problem for these machine translation systems is the variation in orthographic conventions which causes many issues to traditional approaches. Two languages written in two different orthographies are not easily comparable, but orthographic information can also be used to improve the machine translation system. This article offers a survey of research regarding orthography's influence on machine translation of under-resourced languages. It introduces under-resourced languages in terms of machine translation and how orthographic information can be utilised to improve machine translation. We describe previous work in this area, discussing what underlying assumptions were made, and showing how orthographic knowledge improves the performance of machine translation of under-resourced languages. We discuss different types of machine translation and demonstrate a recent trend that seeks to link orthographic information with well-established machine translation methods. Considerable attention is given to current efforts of cognates information at different levels of machine translation and the lessons that can be drawn from this. Additionally, multilingual neural machine translation of closely related languages is given a particular focus in this survey. This article ends with a discussion of the way forward in machine translation with orthographic information, focusing on multilingual settings and bilingual lexicon induction.

==> sota.tex <==

%\citewopar{sennrich-haddow:2016:WMT} included various kinds of linguistic knowledge, such as morpoholgical features, part of speech (POS) tags and syntactic dependency labels, as input features for English-German and English to Romanian NMT systems.

% \citewopar{eriguchi2016} proposed a novel tree-to-sequence NMT model where the encoder processes a tree-based syntactic representation and the attention is able to both address individual tokens and phrases, obtaining improved results for English to Japanese translation.

% \citewopar{GarcaMartnez2016FactoredNM} used a factored NMT model where the system generates lemmas and factors (POS, gender, number, tense, person) for translating from English to French, what leads to an increased vocabulary coverage.

% \citewopar{shi-etal-2016-string} investigated whether the encoder of NMT models learns syntactic information from the source sentence, both when translating from English to French and English to German, generate a linearized constitutional tree from English, and auto-encoding from English to permutated English, finding that different types of syntactic information is captured in different layers.

% \citewopar{niehues-cho-2017-exploiting} used multi-task learning within an encoder-decoder with attention architecture to both translate from German to English and tag POS and recognise named entities in the German sentence, which improved the performance of all individual tasks. Different architectures that shared different components were tested. 

% \citewopar{bastings-etal-2017-graph} explored the use of graph convolutional networks, which do not place any rigid constraint, as encoders for NMT, using syntactic dependency trees for the source language when translating from English to German and Czech. 

% \citewopar{aharoni2017} presented a method to incorporate syntactic information of the target language by using a linearised and lexicalised constituency tree as target language for the NMT system, showing improved word reordering compared to their baseline system on a small-scale human evaluation when translating from German, Czech and Russian to English.

%\citewopar{nadejde2017} introduced CCG supertags within the target word sequence as syntactic information interleaved with the words when translating German and Romanian to English, comparing favourably to multi-task learning.

%\textcolor{gray}{\citewopar{baniata2018} proposed a system that performs three task simultaneously: translating from Arabic Dialects such as Levantine or Maghrebi Arabic to Modern Standard Arabic, translating from Modern Standard Arabic to English, and POS tagging for Arabic Dialects, using word embeddings obtained from FastText. }\tododtr{This paper has several outrageous claims such as achieving perfect translation quality for several languages (page 15)!}

% \citewopar{ataman2018compositional} described the addition of a recurrent neural network to generate compositional representations of the input words, obtaining better results than systems using byte-pair encoding when translating from morphologically rich languages (Arabic, Czech, German, Italian and Turkish) to English. %%

% \citewopar{banerjee-bhattacharyya-2018-meaningless} compared three different approaches for subword units, byte pair encoding, morpheme-based segmentation, and a combination of both, when translating English to Hindi, English to Bengali and Bengali to Hindi.

% \citewopar{etchegoyhen2018} studied NMT, RBMT, and phrase-based statistical machine translation approaches when translating between Basque and Spanish. The authors focus on different subword unit representations, i.e.\ linguistically-motivated or frequency-based word segmentation method. 

%\citewopar{sennrich-haddow:2016:WMT} demonstrated the inclusion of various linguistic knowledge, such as morphological features, part of speech (POS) tags and syntactic dependency labels, as input features for the English-German and English-Romanian NMT systems. \citewopar{baniata2018} proposed a multitask-based NMT system with POS information for translation between English, modern standard Arabic and Arabic dialects, i.e.\ Levantine Arabic and Maghrebi Arabic. The work demonstrated that the POS information for the low resourced Arabic dialects was beneficial for the translation quality, specifically if pre-trained FastText models were injected during the NMT training step. 
%\citewopar{niehues-cho-2017-exploiting} jointly trained several English-German natural language processing tasks in one system with shared encoder and one attention model and decoder per task. By integrating additional linguistic resources via multitask learning, the performance of each individual task was improved.
%%%\citewopar{niehues-cho-2017-exploiting} jointly  training several natural language processing tasks in one system, able to leverage common information and improve the performance of the individual task.  They trained on English-German pair. The goal is to integrate the additional linguistic resources directly into neural models by multi task learning. Common encoder is used for all tasks but separate attention models  and decoders are used. 
% \citewopar{bastings-etal-2017-graph} showed that incorporating syntactic structure such as dependency tree using graph convolutional encoders was beneficial for neural machine translation. Their work focused on exploiting structural information on the source side by adding a second encoder. 
% %. This work creates extra step by creating new encoder.  
% The goal of their work was to provide the encoder with access to rich syntactic information without placing rigid constraints on the interaction between syntax and the translation task

% \citewopar{etchegoyhen2018} studied NMT, RBMT, and phrase-based statistical machine translation approaches for Basque-Spanish. %The authors found optimal configuration in terms of word segmentation and decoding parameter  to improve the results of Neural Machine translation. The  authors explored several large NMT and compared their results with rule base MT and SMT. In our work we utilise rule base system LUCY to improve NMT for Basque-English translation. 
% The authors focus on different subword unit representations, i.e.\ linguistically-motivated or frequency-based word segmentation method. % Our work uses only frequency-based word segmentation. Linguistically motivated segmentation may not available for under-resourced languages. Their work is only on language pair Basque-Spanish. 
% \citewopar{shi-etal-2016-string} investigated whether an encoder-decoder translation system learns syntactic information on the source side as a side affect of training the neural models. Several syntactic labels of the source sentence were created and logistic regression models using the learned sentence encoding vectors or learned word by word hidden vectors were used to predict these syntactic labels.
% %\citewopar{shi-etal-2016-string} investigated whether an encoder-decoder translation system learns syntactic information on the source side as a side affect of training the neural models. Several syntactic labels of the source sentence were created and logistic regression models using the learned sentence encoding vectors or learned word by word hidden vectors were used to predict these syntactic labels.
% %tried to predict these syntactic labels with logistic regression, using the learned sentence encoding vectors or learned word by word hidden vectors. %Find that encoder capture both global and local syntatic information fo the source sentence, and different information tends to be stored at different layers. 
% %Used the hidden states to predict the syntatic labels of sources sentences via logistic regression. English-French and english-German. 
% \citewopar{aharoni2017} presented a method to incorporate syntactic information of the target language in an NMT system, showing improved word reordering compared to their baseline system.
% %showing a better reordering strategy compared to a baseline system. 
% \citewopar{eriguchi2016} proposed an NMT model leveraging syntactic information to improve the accuracy for English$\rightarrow$Japanese translation. The phrase structure of the source sentence was recursively encoded in a bottom-up fashion to first produce a vector representation of the sentence, then decode it while aligning the input phrases and words with the output. \citewopar{bastings-etal-2017-graph} relied on graph-convolutional networks  primarily developed for modelling graph-structured data. These networks used predicted syntactic dependency trees of source sentences to produce representations of words that are sensitive to their syntactic neighbourhoods. \citewopar{nadejde2017} introduced CCG supertags within the target word sequence as syntactic information, processed by the decoder of their NMT system. Their evaluation showed translation quality improvements for the German$\rightarrow$English and Romanian$\rightarrow$English translation directions. Similarly, their approach outperformed multi-tasking approach for the same language pairs. \citewopar{GarcaMartnez2016FactoredNM} trained their NMT model to simultaneously generate the lemma and its corresponding factors, i.e.\ POS, gender, and number, demonstrating that factored architecture increases the vocabulary coverage while decreasing the number of unknown words. \citewopar{ataman2018compositional} described the addition of a recurrent neural network to generate compositional representations of the input words, obtaining better results than systems using byte-pair encoding when translating from morphologically rich languages to English. \citewopar{banerjee-bhattacharyya-2018-meaningless} compared two different approaches for subword units when translating from English to Hindi and Bengali, byte pair encoding and morpheme-based segmentation, showing that the latter approach improves the translations, and further improvements can be achieved by combining both.
